A metric on directed graphs and Markov chains based on hitting probabilities

The shortest-path, commute time, and diffusion distances on undirected graphs have been widely employed in applications such as dimensionality reduction, link prediction, and trip planning. Increasingly, there is interest in using asymmetric structure of data derived from Markov chains and directed graphs, but few metrics are specifically adapted to this task. We introduce a metric on the state space of any ergodic, finite-state, time-homogeneous Markov chain and, in particular, on any Markov chain derived from a directed graph. Our construction is based on hitting probabilities, with nearness in the metric space related to the transfer of random walkers from one node to another at stationarity. Notably, our metric is insensitive to shortest and average walk distances, thus giving new information compared to existing metrics. We use possible degeneracies in the metric to develop an interesting structural theory of directed graphs and explore a related quotienting procedure. Our metric can be computed in $O(n^3)$ time, where $n$ is the number of states, and in examples we scale up to $n=10,000$ nodes and $\approx 38M$ edges on a desktop computer. In several examples, we explore the nature of the metric, compare it to alternative methods, and demonstrate its utility for weak recovery of community structure in dense graphs, visualization, structure recovering, dynamics exploration, and multiscale cluster detection.

==> myfigure.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\fwidth,
height=0.75\fwidth,
at={(0\fwidth,0\fwidth)},
scale only axis,
xmin=0,
xmax=200,
xlabel style={font=\color{white!15!black}},
xlabel={Node},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={Distance},
axis background/.style={fill=white},
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1]
  table[row sep=crcr]{%
1	1.60171325190746e-16\\
2	1.60171325190746e-16\\
3	1.60171325190746e-16\\
4	1.60171325190746e-16\\
5	1.60171325190746e-16\\
6	1.60171325190746e-16\\
7	1.60171325190746e-16\\
8	1.60171325190746e-16\\
9	1.60171325190746e-16\\
10	1.60171325190746e-16\\
11	1.60171325190746e-16\\
12	1.60171325190746e-16\\
13	1.60171325190746e-16\\
14	1.60171325190746e-16\\
15	1.60171325190746e-16\\
16	1.60171325190746e-16\\
17	1.60171325190746e-16\\
18	1.60171325190746e-16\\
19	1.60171325190746e-16\\
20	1.60171325190746e-16\\
21	1.60171325190746e-16\\
22	1.60171325190746e-16\\
23	1.60171325190746e-16\\
24	1.60171325190746e-16\\
25	0\\
26	1.60171325190746e-16\\
27	1.60171325190746e-16\\
28	1.60171325190746e-16\\
29	1.60171325190746e-16\\
30	1.60171325190746e-16\\
31	1.60171325190746e-16\\
32	1.60171325190746e-16\\
33	1.60171325190746e-16\\
34	1.60171325190746e-16\\
35	1.60171325190746e-16\\
36	1.60171325190746e-16\\
37	1.60171325190746e-16\\
38	1.60171325190746e-16\\
39	1.60171325190746e-16\\
40	1.60171325190746e-16\\
41	1.60171325190746e-16\\
42	1.60171325190746e-16\\
43	1.60171325190746e-16\\
44	1.60171325190746e-16\\
45	1.60171325190746e-16\\
46	1.60171325190746e-16\\
47	1.60171325190746e-16\\
48	1.60171325190746e-16\\
49	1.60171325190746e-16\\
50	1.60171325190746e-16\\
51	1.60171325190746e-16\\
52	1.60171325190746e-16\\
53	1.60171325190746e-16\\
54	1.60171325190746e-16\\
55	1.60171325190746e-16\\
56	1.60171325190746e-16\\
57	1.60171325190746e-16\\
58	1.60171325190746e-16\\
59	1.60171325190746e-16\\
60	1.60171325190746e-16\\
61	1.60171325190746e-16\\
62	1.60171325190746e-16\\
63	1.60171325190746e-16\\
64	1.60171325190746e-16\\
65	1.60171325190746e-16\\
66	1.60171325190746e-16\\
67	1.60171325190746e-16\\
68	1.60171325190746e-16\\
69	1.60171325190746e-16\\
70	1.60171325190746e-16\\
71	1.60171325190746e-16\\
72	1.60171325190746e-16\\
73	1.60171325190746e-16\\
74	1.60171325190746e-16\\
75	1.60171325190746e-16\\
76	1.60171325190746e-16\\
77	1.60171325190746e-16\\
78	1.60171325190746e-16\\
79	1.60171325190746e-16\\
80	1.60171325190746e-16\\
81	1.60171325190746e-16\\
82	1.60171325190746e-16\\
83	1.60171325190746e-16\\
84	1.60171325190746e-16\\
85	1.60171325190746e-16\\
86	1.60171325190746e-16\\
87	1.60171325190746e-16\\
88	1.60171325190746e-16\\
89	1.60171325190746e-16\\
90	1.60171325190746e-16\\
91	1.60171325190746e-16\\
92	1.60171325190746e-16\\
93	1.60171325190746e-16\\
94	0.415037499278844\\
95	0.415037499278844\\
96	0.415037499278844\\
97	0.415037499278844\\
98	0.415037499278844\\
99	0.415037499278844\\
100	0.415037499278844\\
101	1\\
102	1\\
103	1\\
104	1\\
105	1\\
106	1\\
107	1\\
108	1\\
109	1\\
110	1\\
111	1\\
112	1\\
113	1\\
114	1\\
115	1\\
116	1\\
117	1\\
118	1\\
119	1\\
120	1\\
121	1\\
122	1\\
123	1\\
124	1\\
125	1\\
126	1\\
127	1\\
128	1\\
129	1\\
130	1\\
131	1\\
132	1\\
133	1\\
134	1\\
135	1\\
136	1\\
137	1\\
138	1\\
139	1\\
140	1\\
141	1\\
142	1\\
143	1\\
144	1\\
145	1\\
146	1\\
147	1\\
148	1\\
149	1\\
150	1\\
151	1\\
152	1\\
153	1\\
154	1\\
155	1\\
156	1\\
157	1\\
158	1\\
159	1\\
160	1\\
161	1\\
162	1\\
163	1\\
164	1\\
165	1\\
166	1\\
167	1\\
168	1\\
169	1\\
170	1\\
171	1\\
172	1\\
173	1\\
174	1\\
175	1\\
176	1\\
177	1\\
178	1\\
179	1\\
180	1\\
181	1\\
182	1\\
183	1\\
184	1\\
185	1\\
186	1\\
187	1\\
188	1\\
189	1\\
190	1\\
191	1\\
192	1\\
193	1\\
};
\addlegendentry{Hitting probability metric}

\addplot [color=mycolor2]
  table[row sep=crcr]{%
1	0.832390969251612\\
2	0.824064476917694\\
3	0.81520414638352\\
4	0.805798451243972\\
5	0.795827586609001\\
6	0.785261629505388\\
7	0.774057864114884\\
8	0.762157369792189\\
9	0.749480988659158\\
10	0.735924804658341\\
11	0.721355246465243\\
12	0.705603844229371\\
13	0.68846149624902\\
14	0.669671801385663\\
15	0.648922528500693\\
16	0.625833507600923\\
17	0.599937875796619\\
18	0.570651079573818\\
19	0.537216798958501\\
20	0.49860689695075\\
21	0.453320982769734\\
22	0.398934133813361\\
23	0.330860860848558\\
24	0.237527000469986\\
25	0\\
26	0.237570598485393\\
27	0.331108554424179\\
28	0.399615072922764\\
29	0.454706221055431\\
30	0.500989226134775\\
31	0.540892484820191\\
32	0.575903269415769\\
33	0.607022253978338\\
34	0.634966913904757\\
35	0.660275132532128\\
36	0.683363167477631\\
37	0.704560545011452\\
38	0.724132375401084\\
39	0.742294385295428\\
40	0.759223515073014\\
41	0.775065691235753\\
42	0.789941722022781\\
43	0.803951894478765\\
44	0.817179637135922\\
45	0.829694485145961\\
46	0.841554507264606\\
47	0.852808306058899\\
48	0.863496672303012\\
49	0.873653954812935\\
50	0.883309193783662\\
51	0.892487056516498\\
52	0.901208607732225\\
53	0.909491941536901\\
54	0.917352697990925\\
55	0.924804483804454\\
56	0.93185921375465\\
57	0.938527386883132\\
58	0.944818309320742\\
59	0.950740273660355\\
60	0.956300703127756\\
61	0.961506267361884\\
62	0.966362975386735\\
63	0.970876250316883\\
64	0.975050989465852\\
65	0.978891612800887\\
66	0.982402102089819\\
67	0.985586032597237\\
68	0.988446598791576\\
69	0.990986635207071\\
70	0.993208633351857\\
71	0.995114755354285\\
72	0.996706844884333\\
73	0.997986435767611\\
74	0.998954758618851\\
75	0.999612745754544\\
76	0.999961034595359\\
77	0.99999996973438\\
78	0.999729603823257\\
79	0.999149697412363\\
80	0.998259717869998\\
81	0.997058837497327\\
82	0.995545930947817\\
83	0.993719572050389\\
84	0.991578030122691\\
85	0.98911926584261\\
86	0.986340926721831\\
87	0.983240342192658\\
88	0.979814518278507\\
89	0.976060131768005\\
90	0.971973523752783\\
91	0.967550692319327\\
92	0.962787284106275\\
93	0.957678584350558\\
94	0.870941920254374\\
95	0.86985906971066\\
96	0.866564019588101\\
97	0.86212474744451\\
98	0.856864547265353\\
99	0.85092190252512\\
100	0.844366825293097\\
101	0.832395115010489\\
102	0.824072850792089\\
103	0.815221055306011\\
104	0.805832503356497\\
105	0.79589568766208\\
106	0.785396104764054\\
107	0.774318433158864\\
108	0.762650096410485\\
109	0.750386519318109\\
110	0.737538088557505\\
111	0.724138457184933\\
112	0.710253453887156\\
113	0.695989547430944\\
114	0.681500630389279\\
115	0.666991849401911\\
116	0.652719321460215\\
117	0.63898482751269\\
118	0.626124966908104\\
119	0.614494807745256\\
120	0.604446799283511\\
121	0.596306598633676\\
122	0.590348375908047\\
123	0.586772836825785\\
124	0.585691301123847\\
125	0.58711845160077\\
126	0.590974863434712\\
127	0.597098541269829\\
128	0.60526304717633\\
129	0.615198911593581\\
130	0.626615049133543\\
131	0.639217647240667\\
132	0.652725059760123\\
133	0.666878247710845\\
134	0.681447049359578\\
135	0.696232978858005\\
136	0.711069400556059\\
137	0.725819896171986\\
138	0.740375519661771\\
139	0.754651481048923\\
140	0.768583651610546\\
141	0.782125155604854\\
142	0.795243213257182\\
143	0.807916324844009\\
144	0.820131832631292\\
145	0.831883861681955\\
146	0.843171617983408\\
147	0.853998009436673\\
148	0.864368549174438\\
149	0.87429049925555\\
150	0.883772214374848\\
151	0.892822648618908\\
152	0.901450992621304\\
153	0.909666413120876\\
154	0.917477871501668\\
155	0.924894002144503\\
156	0.931923035209627\\
157	0.938572751739648\\
158	0.944850461717468\\
159	0.950762997965376\\
160	0.956316720578765\\
161	0.96151752800998\\
162	0.96637087201573\\
163	0.970881774513426\\
164	0.975054845010149\\
165	0.978894297719112\\
166	0.982403967800353\\
167	0.985587326387194\\
168	0.988447494213023\\
169	0.990987253754099\\
170	0.993209059868711\\
171	0.995115048952915\\
172	0.996707046656723\\
173	0.997986574218025\\
174	0.998954853479455\\
175	0.999612810658376\\
176	0.999961078944044\\
177	1\\
178	0.999729624453701\\
179	0.999149711459537\\
180	0.998259727424799\\
181	0.9970588439902\\
182	0.995545935356034\\
183	0.993719575040792\\
184	0.99157803214974\\
185	0.989119267215692\\
186	0.986340927651334\\
187	0.98324034282152\\
188	0.979814518703745\\
189	0.976060132055422\\
190	0.971973523946968\\
191	0.967550692450475\\
192	0.962787284194827\\
193	0.957678584410332\\
};
\addlegendentry{Effective resistance metric}

\end{axis}

\begin{axis}[%
width=1.227\fwidth,
height=0.92\fwidth,
at={(-0.16\fwidth,-0.101\fwidth)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%
